Complex Network Effects on the Robustness of Graph Convolutional Networks

Vertex classification -- the problem of identifying the class labels of nodes in a graph -- has applicability in a wide variety of domains. Examples include classifying subject areas of papers in citation networks or roles of machines in a computer network. Vertex classification using graph convolutional networks is susceptible to targeted poisoning attacks, in which both graph structure and node attributes can be changed in an attempt to misclassify a target node. This vulnerability decreases users' confidence in the learning method and can prevent adoption in high-stakes contexts. Defenses have also been proposed, focused on filtering edges before creating the model or aggregating information from neighbors more robustly. This paper considers an alternative: we leverage network characteristics in the training data selection process to improve robustness of vertex classifiers. We propose two alternative methods of selecting training data: (1) to select the highest-degree nodes and (2) to iteratively select the node with the most neighbors minimally connected to the training set. In the datasets on which the original attack was demonstrated, we show that changing the training set can make the network much harder to attack. To maintain a given probability of attack success, the adversary must use far more perturbations; often a factor of 2--4 over the random training baseline. These training set selection methods often work in conjunction with the best recently published defenses to provide even greater robustness. While increasing the amount of randomly selected training data sometimes results in a more robust classifier, the proposed methods increase robustness substantially more. We also run a simulation study in which we demonstrate conditions under which each of the two methods outperforms the other, controlling for the graph topology, homophily of the labels, and node attributes.

==> related_old.tex <==
\section{Related Work}
\label{sec:related}
Adversarial examples in deep neural networks have received considerable attention since they were documented a few years ago~\cite{Szegedy2014}. Since that time, numerous attack methods have been proposed, largely focused on the image classification domain (though there has been interest in natural language processing as well, e.g.,~\cite{Jia2017}). In addition to documenting adversarial examples, Szegedy et al. demonstrated that such examples can be generated using the limited-memory BFGS (L-BFGS) algorithm, which identifies an adversarial example in an incorrect class with minimal $L_2$ norm to the true data. Later, Goodfellow et al. proposed the fast gradient sign  method (FGSM), where the attacker starts with a clean image and takes small, equal-sized steps in each dimension (i.e., alters each pixel by the same amount) in the direction maximizing the loss~\cite{Goodfellow2015}. Another proposed attack---the Jacobian-based Saliency Map Attack (JSMA)---iteratively modifies the pixel with the largest impact on the loss~\cite{Papernot2016a}. DeepFool, like L-BFGS, minimizes the $L_2$ distance from the true instance while crossing a boundary into an incorrect class, but does so quickly by approximating the classifier as linear, stepping to maximize the loss, then correcting for the true classification surface~\cite{Moosavi-Dezfooli2016}. Like Nettack, these methods all try to maintain closeness to the original data ($L_2$ norm for L-BFGS and DeepFool, $L_0$ norm for JSMA, and $L_\infty$ norm for FGSM).

The Nettack paper only compares to one of these methods: FGSM. In~\cite{Wu2019}, the authors modify JSMA to use integrated gradients and show it to be effective against vertex classification. %In future work, it would be worthwhile to also compare to JSMA and DeepFool. These both have similarities to Nettack: JSMA has a similar greedy strategy of iteratively choosing a dimension to maximally increase the loss, and DeepFool uses a linear approximation of the classifier. While these are evasion rather than poisoning attacks, such a comparison would be worthwhile when evaluating potential defenses.
In addition, new attacks against vertex classification have been introduced, including a method that uses reinforcement learning to identify modifications to graph structure for an evasion attack~\cite{Dai2018} and using meta learning for a global (non targeted) attack~\cite{Zugner2019a}. Exploring the effects of \textsc{StratDegree} and \textsc{GreedyCover} on these methods will be interesting future work.

Defenses to attacks such as FGSM and JSMA have been proposed, although several prove to be insufficient against stronger attacks. Defensive distillation is one such defense, in which a classifier is trained with high ``temperature'' in the softmax, which is reduced for classification~\cite{Papernot2016}. While this was effective against the methods from~\cite{Szegedy2014,Goodfellow2015, Papernot2016a,Moosavi-Dezfooli2016}, it was shown in~\cite{Carlini2017} that modifying the attack by changing the constraint function (which ensures the adversarial example is in a given class) renders this defense ineffective. More defenses have been proposed, such as pixel deflection~\cite{Prakash2018} and randomization techniques~\cite{Xie2018}, but many such methods are still found to be vulnerable to attacks~\cite{Athalye2018,Athalye2018a}. Future work will also consider defenses that appear promising (e.g.,~\cite{Wong2018, Croce2019}) if they can be applied in the graph domain. More recent work has focused on robustness of GCNs, including work on robustness to attacks on attributes~\cite{Zugner2019b} and more robust variants of the GCN~\cite{Zhu2019}. In particular, evaluating the impact of \textsc{StratDegree} and \textsc{GreedyCover} on certifiable robustness as outlined in~\cite{Bojchevski2019b} will be important future work. Finally, attacks against classifiers other than GCNs~\cite{Yu2018} and objectives other than vertex classification---such as node embedding~\cite{Bojchevski2019a} and community detection~\cite{Kegelmeyer2018}---would be interesting to consider, to determine whether any strategy works against many adversary tactics. 

==> table.tex <==
\begin{table*}
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
        \hline
        Dataset & Thres. &\%ile& 10\% & 15\%& 20\% & 25\%& 30\% & \textsc{StratDegree}&\textsc{GreedyCover}\\
        \hline
        \hline
        \multirow{3}{*}{CiteSeer} & \multirow{3}{*}{0} & 20& 1.50 (0.17)
        & 2.87 (0.72)
        & 2.25 (0.40)
        & 2.95 (0.75)
        & 1.99 (0.29)
        & \textbf{4.02} (0.56)
        & 3.84 (0.47)\\
        \cline{3-10}
        & & 50& 3.39 (0.53)
        & 6.88 (0.81)
        & 6.65 (0.53)
        & 6.14 (1.01)
        & 6.68 (1.06)
        & \textbf{10.88} (2.00)
        & 8.69 (1.61)\\
        \cline{3-10}
        & & 80
        & 12.53 (2.04)
        & 19.75 (2.63)
        & 15.01 (1.70)
        & 17.75 (2.61)
        & 14.89 (2.61)
        & \textbf{41.04} (4.50)
        & 27.86 (4.34)\\
        \hline
        \multirow{3}{*}{Cora} & \multirow{3}{*}{0}  &20& 2.00 (0.36)
        & 2.27 (0.35)
        & 2.90 (0.70)
        & 2.08 (0.17)
        & 3.44 (0.44)
        & \textbf{3.50} (0.71)
        & 3.00 (0.53)\\
        \cline{3-10}
        & & 50 & 5.22 (0.85)
        & 5.64 (0.12)
        & 9.19 (1.36)
        & 5.48 (0.47)
        & 8.52 (0.87)
        & \textbf{10.92} (2.03)
        & 9.20 (1.17)\\
        \cline{3-10}
        & & 80& 13.84 (1.24)
        & 13.64 (1.01)
        & 18.25 (1.76)
        & 14.88 (1.15)
        & 21.45 (2.50)
        & \textbf{29.34} (6.36)
        & 17.02 (2.71)\\
        \hline
        \multirow{3}{*}{PolBlogs} & \multirow{3}{*}{$\ln{1.5}$}&20& 1.13 (0.63)
        & 1.90 (1.09)
        & 1.07 (0.46)
        & 2.69 (0.64)
        & \textbf{3.76} (2.05)
        & 0.28 (0.15)
        & 1.72 (0.86)\\
        \cline{3-10}
        & & 50& 41.89 (5.03)
        & 20.00 (10.95)
        & 22.95 (8.89)
        & 34.51 (8.82)
        & 40.16 (6.31)
        & 0.71 (0.29)
        & \textbf{50.00} (0.00)\\
        \cline{3-10}
        & & 80& \textbf{50.00} (0.00)
        & 40.32 (8.66)
        & 30.00 (10.95)
        & 40.77 (8.26)
        & \textbf{50.00} (0.00)
        & 34.87 (8.97)
        & \textbf{50.00} (0.00)\\
        \hline
    \end{tabular}
    \caption{Budget required for an adversary to achieve a given level of attack success, varying training set selection method and amount of training data. Values are the average (with standard error) number of perturbations required for the attacker to succeed the specified proportion of the time. While more randomly selected training data typically improves performance, it does not do so consistently, nor does it reliably perform better than \textsc{StratDegree} and \textsc{GreedyCover}. Note that 50 perturbations is the maximum attempted in all cases, and assigned as the required budget when no level of perturbation succeeds.}
    \label{tab:varySize}
\end{table*}
